Automatic Non-Invasive Isolation of Respiratory Cycles

In this paper, we introduce a novel algorithm designed to isolate individual respiratory cycles on a thoracic respiratory inductance plethysmography signal. The algorithm locates breaths using signal processing and statistical methods and enables the analysis of sleep data on an individual breath level. The algorithm was evaluated on 7.3 hours of hand-annotated data, or 8782 individual breaths in total, and was estimated to correctly isolate 94% of respiratory cycles while producing false positives that amount to only 5% of the total number of detections. The algorithm was specifically evaluated on data containing a great number of sleep-disordered breathing events. We found that the algorithm did not suffer in terms of accuracy when detecting breaths in the presence of sleep-disordered breathing. The algorithm was also evaluated across a large set of participants, and we found that the accuracy of the algorithm was consistent across participants. This algorithm is finally made public via an open-source Python library.

==> Sections/Background.tex <==
% \section{Background}
% Currently, the field of doing BSS is mainly rooted in statistical methods with the most frequently used methods being peak and valley detections.

% ABCD et.al. \cite{123} used some methods to do this, but failed in doing xyz .

% The field of BSS is varied in terms of approaches as described above, and there is significant need of some study comparing and evaluating the existing approaches of automatically performing BSS. 

==> Sections/Conclusion.tex <==
\section{Conclusion}
This paper introduces BreathFinder, a novel algorithm designed to find individual breaths in the thoracic RIP signal. The algorithm uses periodicity estimation and sine fitting procedures to pinpoint the locations of individual breaths within a PSG.

The algorithm was evaluated on approximately 7.8 hours of manually annotated breathing intervals. The results suggest that the algorithm detects on average 94\% of breaths correctly, and of the detected breaths, only 4\% on average being false positives. The placement error of the correctly detected breaths was generally within acceptable margins, being less than 10\% of the mean breath length. 

The exceptional performance of the algorithm in terms of the evaluation metrics suggests that it is usable for further analysis of sleep data on a breath by breath basis. The evaluation has the drawbacks that it is only formally done on the thoracic RIP signal, and the evaluation was only done on data from one dataset. The algorithm has furthermore only been evaluated against a RIP signal using 25 as the sampling frequency.

% \subsection{Future work}

